CCPL: Contrastive Coherence Preserving Loss for Versatile Style Transfer

In this paper, we aim to devise a universally versatile style transfer method capable of performing artistic, photo-realistic, and video style transfer jointly, without seeing videos during training. Previous single-frame methods assume a strong constraint on the whole image to maintain temporal consistency, which could be violated in many cases. Instead, we make a mild and reasonable assumption that global inconsistency is dominated by local inconsistencies and devise a generic Contrastive Coherence Preserving Loss (CCPL) applied to local patches. CCPL can preserve the coherence of the content source during style transfer without degrading stylization. Moreover, it owns a neighbor-regulating mechanism, resulting in a vast reduction of local distortions and considerable visual quality improvement. Aside from its superior performance on versatile style transfer, it can be easily extended to other tasks, such as image-to-image translation. Besides, to better fuse content and style features, we propose Simple Covariance Transformation (SCT) to effectively align second-order statistics of the content feature with the style feature. Experiments demonstrate the effectiveness of the resulting model for versatile style transfer, when armed with CCPL.

==> intro_backup.tex <==
% \section{Introduction}


% We humans are always fascinated by the beauty of what we see or imagine. In the past, it takes hours or even days for an expert to produce an artistic imagery. Now with the development of artistic style transfer, we can easily create a hybrid image with the structure of one input and the feel of the other input. Gatys $et~al.$~\cite{gatys2016image} first introduced Deep Neural Networks (DNNs) to the field of style transfer. Since then, a variety of approaches tried to use feed-forward networks to reduce the inference time~\cite{johnson2016perceptual,ulyanov2016texture} and transfer arbitrary style within a single model~\cite{chen2016fast,sheng2018avatar,huang2017arbitrary,li2017universal}. Compared with these former algorithms, recent image style transfer methods~\cite{li2019learning,hong2021domain,chen2021artistic} made considerable efforts to preserve the fidelity of the content sources without degrading stylization. There are also some researches focusing on photo-realistic style transfer~\cite{yoo2019photorealistic,an2019stylenas,hong2021domain} and stereoscopic style transfer~\cite{chen2018stereoscopic,yin20213dstylenet}.

% Nowadays, people are not content with creating fascinating images only. We are also interested in rendering videos. For video style transfer, it is of vital importance to maintain the temporal consistency of the source videos. Former methods~\cite{ruder2016artistic,chen2017coherent,gupta2017characterizing,huang2017real,ruder2018artistic,gao2018reconet} used optical flow as guidance to restore estimated motions of the original videos. However, optical flow estimation is time-consuming and not perfectly accurate, which could result in severe artifacts in the generated videos. In consideration of these issues, recently, some algorithms~\cite{li2019learning,deng2020arbitrary,liu2021adaattn} tried to improve the temporal consistency of the video outputs with single-frame regularizations. By linearly stylizing the video frames independently, the coherence of the original video is naturally inherited, thus leading to better stability in the generated video. However, although linear transformation is performed in the deep layer of the feature maps, without explicitly guiding, the linearity is largely affected by the non-linear decoder and global optimization loss functions. Therefore, existing single-frame-based algorithms are less effective to produce stable video outputs. 

% \begin{figure}[t]
% \centering
% \includegraphics[width=1.0\textwidth]{Fig. 1.pdf} % Reduce the figure size so that it is slightly narrower than the column.
% \caption{On the upper side of the figure, we show two consecutive frames of a stable video and their stylized results. We show a random patch of the former frame in the red box and a corresponding patch (same location) of the latter frame in the blue box. The mutual information of differences of these patches is encouraged to be maximized between the original and stylized frames to preserve the coherence of the source video. In the lower half of the figure we show examples of existing algorithms (AdaIN~\cite{huang2017arbitrary}, SANet~\cite{park2019arbitrary},  Linear~\cite{li2019learning}) training with or without our CCP loss.}
% \label{fig1}
% \end{figure}

% In this work, we devise a generic loss named~\textbf{Contrastive Coherence Preserving (CCP)} loss to improve the temporal consistency of the stylized videos without degrading stylization. For stable videos, when we focus on a random area, the local patches of the video frames should be temporally consistent, which means the changes among these patches are smooth and consistent. Our goal is to preserve the coherence in the stylized videos. (However, stable video datasets are rare and hard to obtain. ...) We note that adjacent frames of a stable video are usually closely-related, with only slight shifts or minor changes in scale. Therefore in most cases, a random local patch of the current frame can be found in the neighbor area of the previous frame (the patches in the blue boxes shown in Fig.~\ref{fig1}). Enlightened by this, in this work, we consider the differences between patches and their near neighbor patches within the same images as a substitute for corresponding patches of stable videos. And instead of forcing the corresponding pairs to be identically the same, which is a too strict restriction that prevents the image from changing, our proposed CCP loss adopts InforNCE loss~\cite{oord2018representation} as a looser constraint to maximize the mutual information of them. Besides, we only sample patches of a certain number for one time. Benefit from iterative training, the affinity among all neighboring patches can be preserved while the computation costs reduce significantly. With our setting, we note that the temporal consistency of the video outputs improves significantly while the stylization remains satisfying (see Fig.~\ref{fig4} and Fig.~\ref{fig5}). Besides, since the semantic information of the content sources has been preserved better, the visual quality of the stylized images is even better (see Fig.~\ref{fig1} and Fig.~\ref{fig6}). 

% Our proposed CCP loss has no requirements for the network structure and it only needs images as training data. Therefore we can apply it to any existing image style transfer networks during training to improve their performance on images and videos (see Fig.~\ref{fig1} and Table.~\ref{table1}). For better feature migration, we also propose~\textbf{Simple Covariance Transformation (SCT)} to align second-order statistics of content and style features effectively. Our contributions can be summarized as follows:

% \begin{enumerate}
%     \item We propose Contrastive Coherence Preserving (CCP) loss to improve the temporal consistency of the generated videos without hurting stylization. It is effective and transferable to other learning-based image style transfer networks.
%     \item We propose Simple Covariance Transformation (SCT) to align second-order statistics of content and style features effectively.
%     \item Our proposed SCT is simpler and more effective than other SOTA methods (about 20 to 30 frames per second at the scale of $512\times512$), which is more practically useful for real-world scenarios.
%     \item We also apply our CCP loss to other tasks such as photo-realistic style transfer and image-to-image translation. The results are comparable to SOTAs without the need for extensive modification.
% \end{enumerate}
